FogGuard: guarding YOLO against fog using perceptual loss

In this paper, we present FogGuard, a novel fog-aware object detection network designed to address the challenges posed by foggy weather conditions. Autonomous driving systems heavily rely on accurate object detection algorithms, but adverse weather conditions can significantly impact the reliability of deep neural networks (DNNs). Existing approaches include image enhancement techniques like IA-YOLO and domain adaptation methods. While image enhancement aims to generate clear images from foggy ones, which is more challenging than object detection in foggy images, domain adaptation does not require labeled data in the target domain. Our approach involves fine-tuning on a specific dataset to address these challenges efficiently. FogGuard compensates for foggy conditions in the scene, ensuring robust performance by incorporating YOLOv3 as the baseline algorithm and introducing a unique Teacher-Student Perceptual loss for accurate object detection in foggy environments. Through comprehensive evaluations on standard datasets like PASCAL VOC and RTTS, our network significantly improves performance, achieving a 69.43\% mAP compared to YOLOv3's 57.78\% on the RTTS dataset. Additionally, we demonstrate that while our training method slightly increases time complexity, it doesn't add overhead during inference compared to the regular YOLO network.

==> tex/report.tex <==

\begin{itemize}
\item Detecting all weather conditions in an image
\begin{itemize}
\item Most methods try to remove them, but we are trying to extract information
about the level of adversity from them
\item Most methods try to detect each weather condition separately and fine-tune
each model to achieve an excellent performance, that results to a very
complicated model. We are combining all together.
\item A few architectures have been proposed to deal with image restoration. But,
they are fine-tuned for individual datasets
\end{itemize}
\item Detecting the severity of a weather condition in the network to assess the
risk of relying on the results of network
\item Using YOLO-v3, we are modifying the network and the loss function in a way to
encourage weather condition detection
\item Given the weather condition causes a distortion in an image, can we use
perceptual loss to encourage detecting weather conditions in the inner layers
of the network?
\end{itemize}

\section{Problem Statement}
\label{sec:org987d06a}
In many real-world scenarios, object detection in adverse weather conditions is
essential for tasks such as surveillance, autonomous driving, and
robotics. However, adverse weather conditions such as rain, fog, and snow can
make object detection challenging due to the degradation of visual quality and
the loss of image details. Traditional image processing techniques and filters
often fail to remove these weather conditions, making it difficult to detect
objects accurately. Therefore, we propose a solution to overcome these
challenges using a novel approach that leverages the strength of  YOLO-v3 object
detection network that can detect weather conditions
from images and assess the risk and uncertainty involved in the network's object
detection results. 

Let us assume we have a dataset of n images of size \(h \times w\) captured
in adverse weather conditions, denoted by \(X = {x_1, x_2, ..., x_n}\). Each
image \(x_i\) is labeled with a ground truth object detection bounding box,
denoted by \(y_i\). 

We use a modified version of YOLO-v3 network as our object detection model to
remove weather conditions. The network consists of \(L\) layers, with each layer
\(l\) performing a set of convolutional operations, batch normalization, and
activation function on the input feature map \(F_l\) to produce an output feature
map \(F_{l+1}\). We denote the parameters (weights, biases) of layer \(l\) as \(w_l\) and
\(b_l\). 

We define a loss function \(L_o\) that trains the network to perform accurate object
detection on the images after removing the weather conditions. We can use the
YOLO-v3 loss function that combines localization and confidence loss. The loss
for the i-th image can be denoted by \(L_o(x_i, y_i, w_l, b_l)\). 


Now, let's define a loss function that penalizes the network for not detecting
the weather condition features in that layer. One way to do this is to use a
feature reconstruction loss, which compares the reconstructed feature maps in
layer l with the original input images with the weather conditions.

Let \(F_l(x_j, w_l)\) be the feature map of layer l given the input image \(x_j\) and
network parameters \(w_l\). Let \(\hat{x}_j\) be the reconstructed image given the feature
map \(F_l(x_j, w_l)\) and the network parameters \(w_l\). We can define the feature
reconstruction loss as: 

$$
L_f(x_j, w_l) = || x_j - \hat{x}_j ||^2
$$

where \(||.||^2\) denotes the L2-norm of the difference between the input image and its reconstruction.

By minimizing the feature reconstruction loss, the network is encouraged to
reconstruct the input image without the weather condition features. As a side
effect, the network is also encouraged to detect the weather condition features
in layer l because removing them is necessary for good reconstruction. 

You can add this feature reconstruction loss to the object detection loss function as a regularization term. The total loss function can be defined as:
$$
L_{total}(x_j, y_j, w_l, b_l) = L_o(x_j, y_j, w_l, b_l) + \lambda * L_f(x_j, w_l)
$$

where \(\lambda\) is a hyperparameter that controls the strength of the
regularization. By tuning lambda, you can adjust the balance between object
detection accuracy and weather condition detection in layer l.

We optimize the network parameters \(w_l\) and \(b_l\) with respect to the total loss using stochastic gradient descent (SGD) or ADAM optimizer. The optimization problem can be formulated as

$$
   \min_{w_l, b_l} [1/n * \sum_i^n L_{total}(x_i, y_i, w_l, b_l)]
$$

Overall, using this mathematical notation and equations can help you specify the problem, solution, and evaluation metrics of your proposed method clearly and concisely.

\textbf{Perceptual loss} is a term in the loss function that encourages natural and
perceptually pleasing results. 

\textbf{Feature-wise losses}:
A new category of loss functions, which has recently gained noticeable
popularity, employs neural networks as feature extractors. Most commonly, the
loss is computed as the L2 distance between the activations of the hidden layers
of a trained image classification network.
\subsection{Perceptual Loss}
Intuition behind using perceptual loss rather than regular loss
\subsection{Teacher-Student Architecture}
Knowledge Distillation and why it's used in this problem?

